Navigating Image Restoration with VAR's Distribution Alignment Prior

Generative models trained on extensive high-quality datasets effectively capture the structural and statistical properties of clean images, rendering them powerful priors for transforming degraded features into clean ones in image restoration. VAR, a novel image generative paradigm, surpasses diffusion models in generation quality by applying a next-scale prediction approach. It progressively captures both global structures and fine-grained details through the autoregressive process, consistent with the multi-scale restoration principle widely acknowledged in the restoration community. Furthermore, we observe that during the image reconstruction process utilizing VAR, scale predictions automatically modulate the input, facilitating the alignment of representations at subsequent scales with the distribution of clean images. To harness VAR's adaptive distribution alignment capability in image restoration tasks, we formulate the multi-scale latent representations within VAR as the restoration prior, thus advancing our delicately designed VarFormer framework. The strategic application of these priors enables our VarFormer to achieve remarkable generalization on unseen tasks while also reducing training computational costs. Extensive experiments underscores that our VarFormer outperforms existing multi-task image restoration methods across various restoration tasks.

==> 0_abstract.tex <==
\begin{abstract} 
Generative models trained on extensive high-quality datasets effectively capture the structural and statistical properties of clean images, rendering them powerful priors for transforming degraded features into clean ones in image restoration. 
VAR, a novel image generative paradigm, surpasses diffusion models in generation quality by applying a next-scale prediction approach. 
It progressively captures both global structures and fine-grained details through the autoregressive process, consistent with the multi-scale restoration principle widely acknowledged in the restoration community. 
Furthermore, we observe that during the image reconstruction process utilizing VAR, scale predictions automatically modulate the input, facilitating the alignment of representations at subsequent scales with the distribution of clean images.
To harness VAR's adaptive distribution alignment capability in image restoration tasks, we formulate the multi-scale latent representations within VAR as the restoration prior, thus advancing our delicately designed VarFormer framework.
The strategic application of these priors enables our VarFormer to achieve remarkable generalization on unseen tasks while also reducing training computational costs.
Extensive experiments underscores that our VarFormer outperforms existing multi-task image restoration methods across various restoration tasks. The code is available at 
https://github.com/siywang541/Varformer.

\end{abstract}

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[!ht]
\centering 
{\includegraphics[width=0.9\linewidth]{figs/fig1_4.pdf}}
\caption{Motivation of VarFormer. (1) As the autoregressive scale evolves, VAR's multi-scale representations shift focus from 
capturing global patterns at lower scales to highlighting fine-grained details at higher scales. 
(2) VAR's scale predictions adaptively modulate the input to align with the distribution of clean images. 
Utilizing VAR's alignment prior on varied scale features related to degradation types allows us to eliminate associated degradations. 
} 
\label{fig:m_comp}
\end{figure}


Image restoration (IR) aims to reconstruct a high-quality (HQ) image from its degraded low-quality (LQ) counterpart, making it widely applicable in various real-world scenarios, including photo processing, autonomous driving, and surveillance. 
Recent advances in deep learning have led to powerful IR approaches that excel at addressing specific types of degradation, such as denoising~\cite{wang2023lg,zhang2017beyond,zhang2022practical}, deblurring~\cite{quan2023neumann,ruan2022learning,tsai2022stripformer}, and low-light enhancement~\cite{guo2020zero,wu2023learning,xu2023low}, etc. 
However, these task-specific models struggle with the varied and unpredictable degradations commonly present in real-world scenarios, emphasizing the need for a generalist approach capable of restoring multiple types of degradation.

\begin{figure*}[ht]
\centering 
\includegraphics[width=0.8\linewidth]{figs/fig2_add_tb.pdf}
% \vspace{-0.5em}
\caption{Illustration of our investigation about the multi-scale distribution alignment priors within VAR. 
(a) Reconstruction Training: To ensure the coherence of teacher-forcing-based autoregressive predictions, we employ cross-attention to inject multi-scale embeddings ${F}_{e}$ obtained from the VQVAE encoder into the scale autoregression Transformer in VAR~\cite{tian2024visual} for image reconstruction pre-training. 
During this process, we freeze the VAR and train only the cross-attention mechanism using clean images. 
(b) Reconstruction Testing: We feed degraded images into the trained VAR to obtain outputs from the VQVAE encoder, denoted as ${F}_{e}^{deg}$, and the multi-scale predictions from the VAR Transformer, denoted as ${F}_{v}^{deg}$. 
(c-d) Observation: By partially replacing ${F}_{e}^{deg}$ with ${F}_{v}^{deg}$ and mapping the modified multi-scale features back to the pixel space through the decoder, the disappearance of various degradations occurs when replacing different scale features, demonstrating a transition from capturing global information at lower scales to focusing on fine-grained details at higher scales. 
} 
\label{fig2}
\end{figure*}

Recently, several pioneers have sought to develop a universal image restoration model, making considerable strides in the field.
MPRNet~\cite{Zamir2021MultiStagePI} designs a multi-stage architecture that progressively learns image restoration functions for various known degradations.  
AirNet~\cite{Li2022AllInOneIR} distinguishes various image degradation in latent space through a contrastive-based degraded encoder. 
IDR~\cite{zhang2023ingredient} adopts an ingredients-oriented paradigm to investigate the correlation among various restoration tasks. 
However, given the infinite possible solutions for each degraded image, relying exclusively on the degraded image as the sole feature source while neglecting the prior distribution of clean images represents a major limitation for these models in terms of structural reconstruction and realistic texture restoration.



To alleviate these limitations, some studies has focused on the impact of generative priors within the image restoration (IR) community. 
These investigations are grounded in the characteristic that generative models inherently learn high-quality image reconstruction, enabling them to maintain robust high-quality priors that facilitate the transition of degraded features to the clean domain. 
These approaches perform IR tasks using the generative prior~\cite{kawar2022denoising,lin2023diffbir,wang2022zero} from the GAN or diffusion models, achieving superior performance and demonstrating the effectiveness of generative prior for IR tasks.
Recently, a novel generative paradigm, VAR, stands out in the image generation community, recognized for its efficiency and generation capabilities that surpass those of Stable Diffusion~\cite{tian2024visual} .
VAR generates images with progressively increasing resolutions by utilizing marker mapping for next-scale predictions, resolving the conflict between the inherent bidirectional and two-dimensional structural correlations in image patch labeling and the unidirectional nature of the autoregressive model. 

Motivated by the powerful generative capabilities of VAR and the alignment between its endogenous scale representation and the widely recognized multi-scale restoration principle, we aim to explore the rich prior knowledge embedded in the pre-trained VAR across the scale dimension for restoration tasks.
Our investigation reveals the adaptability of the autoregressive scale representation, as the VAR feature representation shifts from capturing wide-ranging global patterns at lower scales to highlighting intricate details at higher scales. 
As described in Fig.~\ref{fig2} a and b, we apply pre-trained VAR to reconstruct the paired clean and degraded images, respectively. 
When we replace the partially scale features of the degraded images obtained from the VQVAE encoder with the autoregressive generated scale features, the degradation of the images gradually diminishes.
Specifically, Fig.~\ref{fig2} c shows that substituting lower scales can alleviate global degradations (\emph{e.g.}, low light and haze), while higher scales address local degradations (\emph{e.g.}, noise and rain). 
For a boarder investigation, we further perform a statistical analysis of the prior knowledge related to high-quality images, utilizing 100 paired images for each type of degradation. 
As illustrated in Fig.~\ref{fig:tsne}
, VAR's next-scale prediction projects the multi-scale latent representations of both degraded and clean images into a common space, thereby reducing the distribution gap between various degradations and clean images, demonstrating the model's adaptive distribution alignment capability.

Building on the above observation, we develop a novel framework, named  VarFormer, which integrates multi-scale distribution alignment priors from VAR to restore various degradation types within a single model.
Specifically, to adaptively incorporate the valuable VAR scale priors associated with specific degradation types, we design the Degradation-Aware Enhancement (DAE) module that distinguishes different degradation types and filters out unnecessary interference, thereby providing effective guidance for the restoration process.
Then, to alleviate structural warping and textural distortion resulting from the fusion of high-quality priors and low-quality degraded features, we present the Adaptive Feature Transformation (AFT) module. 
Furthermore, we employs an adaptive mixing strategy to effectively incorporate low-level features from the encoder, enhancing image details while mitigating potential information loss incurred by downsampling operations.
By integrating these designs, our VarFormer not only captures a high-quality feature distribution that enables exceptional generalization on unseen tasks but also accelerates convergence, thus reducing training computational costs.

Our contributions are summarized as follows:

\begin{itemize}
    \item We investigate the multi-scale representations of VAR and reveal its endogenous multi-scale distribution alignment priors, which transition from capturing global color information to focusing on fine-grained details, adaptively aligning the input images with clean images scale by scale as the autoregressive scale evolves.
    \item We propose the VarFormer framework integrated with multi-scale priors for multiple degradation restoration, embracing generalization capability on unseen tasks. To the best of our knowledge, this is the first attempt to explore generative priors from VAR for image restoration. 
    \item Extensive experiments on six image restoration tasks demonstrate the efficiency and effectiveness of VarFormer, including deraining, deblurring, dehazing, low-light image enhancement, Gaussian and real denoising. 
\end{itemize}




==> 2_related_work.tex <==
\section{Related Work}
\label{sec:Relate}
\subsection{Image Restoration}
The purpose of image restoration is to reconstruct high quality natural images from the degraded images (e.g. noise, blur, rain drops).
Early methods typically focuses on incorporating various natural image priors along with hand-crafted features for specific degradation removal tasks~\cite{Babacan2009VariationalBB,he2010single}. Recently, deep learning based methods have made compelling progress on various image restoration tasks. For instance, 
DGUNet is proposed based on Proximal Gradient Descent (PGD) algorithm for a gradient estimation strategy without loss of interpretability~\cite{mou2022deep}.
IDR~\cite{zhang2023ingredient} employs an ingredients-oriented paradigm to investigate the correlation among various restoration tasks. TransWeather~\cite{valanarasu2022transweather} designs a transformer-based network with learnable weather type queries to tackle various weather degradation. 


\subsection{Generative Priors in Image Restoration}
The generative models trained on clean data excel at capturing the inherent structures of the image, enabling the generation of images that follow natural image distribution, which helps boost the performance in many low-level vision tasks. Generative Priors of pretrained GANs~\cite{brock2018large,karras2017progressive,karras2019style,karras2020analyzing} is previously exploited by GAN inversion~\cite{abdal2019image2stylegan,gu2020image,gu2020image} , whose primary aim is to find the closest latent codes given an input image. Beyond GANs, Diffusion models have also been effectively used as generative priors in IR ~\cite{kawar2022denoising,lin2023diffbir,wang2024exploiting,wang2022zero}, pushing the frontiers of advanced IR. Our work primarily focuses on generative priors derived from VAR~\cite{tian2024visual}, which has never been explored before.






==> 3_method.tex <==
\section{Method}
\label{sec:method}

In this section, we provide a detailed introduction to our method. We first investigate the properties of VAR at different scales in Sec.~\ref{sec:3.1}. And then, we provide a detailed introduction to the structural design of VarFormer in Sec.~\ref{sec:3.2}.


\subsection{Generative Priors in VAR for IR}
\label{sec:3.1}
Different from traditional autoregressive methods, VAR introduces a novel visual autoregressive modeling paradigm, shifting from "next-token prediction" to "next-scale prediction". This paradigm can solve mathematical inconsistencies and structural degradation, which is more optimal for generating highly-structured images. In VAR, each unit predicts an entire token map at a different scale. Starting with a 1 × 1 token map ${r}_{1}$, VAR predicts a sequence of multi-scale token maps $({r}_{1}, {r}_{2},\dots,{r}_{K})$, increasing in resolution. The generation process is expressed as:
\begin{equation}
p({r}_{1}, {r}_{2},\dots,{r}_{K}) = \displaystyle\prod_{k=1}^{K}p( {r}_{k}| {r}_{1}, {r}_{2},\dots,{r}_{k-1})
\end{equation}

where ${r}_{k} \in {[V]}^{{h}_{k} \times {w}_{k}}$ represents the token map at scale $k$, with dimensions ${h}_{k}$ and ${w}_{k}$, conditioned on previous maps $({r}_{1}, {r}_{2},\dots,{r}_{k-1})$. Each token in ${r}_{k}$ is an index from the VQVAE codebook $V$, which is trained through multi-scale quantization and shared across scales.

To explore the information that VAR focuses on at different scales, we need it to model specific images. First, we obtain GT index sequence ${F}_{e}^{cle} = {[{F}_{{e}_{i}}^{cle}]}_{i=1}^{N}$ at various scales and provide them to VAR. To maintain the continuity and controllability of the VAR modeling process, we inject ${F}_{e}^{cle}$ into the transformer using cross-attention. Finally, we decode the predicted sequence ${F}_{v}^{cle}$ back to the pixel space. The pipeline is shown in Fig.~\ref{fig2}. Please note that the reconstruction training process is conducted only on clean images, with all modules except the cross-attention module being frozen.
Following that, we replace the clean images with degraded images to obtain the GT index sequence ${F}_{e}^{deg} = {[{F}_{{e}_{i}}^{deg}]}_{i=1}^{K}$ and the sequence ${F}_{v}^{deg}$ predicted by the Transformer. To explore the information that VAR focuses on at various scales, we replace the corresponding ${F}_{e}^{deg}$ sequence with the specific scale sequence from ${F}_{v}^{deg}$,Then, we decode the new sequence back into the image space. The process can be mathematically formulated as:
\begin{equation}
 {I}_{rec} = D(\displaystyle\sum_{i\notin C}^{K}{F}_{{e}_{i}}^{deg} + \displaystyle\sum_{i\in C}^{K}{F}_{{v}_{i}}^{deg})
\end{equation}
where $D$ denotes the VAR Decoder, $C$ refers to the set of indices that need to be replaced. In Fig.~\ref{fig2}, it can be observed that VAR features at different scales naturally restore different types of typical degradation. 
Specifically, substituting lower scales can alleviate global degradations (\emph{e.g.}, low light and haze), while higher scales address local degradations (\emph{e.g.}, noise and rain). Furthermore, as shown in Fig.~\ref{fig:tsne}, by comparing the t-SNE diagrams of the latent representations ${F}{e}$ from the VQVAE encoder and ${F}_{v}$ from the scale autoregression Transformer on various degraded images, the capability of VAR in effectively aligning distributions is demonstrated.
Therefore, the reasonable combination of VAR features at different scales as priors can be beneficial to the image restoration process.



\subsection{Architecture of the VarFormer}
\label{sec:3.2}
Based on the observations from Sec.~\ref{sec:3.1}, we propose VarFormer, which leverages the multi-scale distribution alignment priors in VAR to facilitate image restoration. As shown in Fig.~\ref{fig3}, the VarFormer training process is divided into two stages. The first stage is dedicated to extracting the priors from VAR, while the second stage utilizes these priors to guide the restoration process. {\bf In the first stage}, the model is enhanced with an Adapter module on top of the VAR that has been finetuned for reconstruction in Sec.~\ref{sec:3.1}. {\bf In the second stage}, the model incorporates Degradation-Aware Enhancement (DAE) modules and Adaptive Feature Transformation (AFT) modules, which integrate the multi-scale distribution alignment priors extracted in the first phase to accomplish image restoration.

{\bf Adapter for Domain Shift} (Train in Stage 1).
Due to the existence of distributional shift between high quality sources for VAR pre-training and degraded datasets for image restoration, direct reuse of the features from the Encoder of VAR may be suboptimal. However, fine-tuning disrupts the the knowledge in VAR. Therefore, inspired by AWRCP~\cite{ye2023adverse}, we chose to freeze the encoder and insert an Adapter containing self-attention blocks after it to retain pre-trained knowledge while narrowing the domain gap.

 \begin{figure}[ht]
\centering 
{\includegraphics[width=0.9\linewidth]{figs/fig_tsne_h.pdf}}
\caption{
The t-SNE diagrams demonstrate that VAR's next-scale prediction can reduce the gap between degraded and clean images, effectively aligning their distributions.
} 
\label{fig:tsne}
\end{figure} 

{\bf Degradation-Aware Enhancement (DAE)} (Train in Stage 2).
To address various degradation tasks by appropriately combining information at different scales, we propose Degradation-Aware Enhancement (DAE). An illustration of DAE is shown in Fig.~\ref{fig3}. 
After reconstruction pre-training on extensive clean images, the encoder of VAR has developed the capability to discern what level of information each network layer should focus on. Consequently, we can use the outputs ${F}_{{e}_{v}}$ from its different layers to determine the weights for scale priors. Specifically, for the $i$-th layer of the encoder or decoder in the second stage, we take ${F}_{{e}_{v}}^{i}$ as the input for the weight predictor within the DAE. After processing through Swin-transformer blocks that mitigate the impact of image content and a projection convolutional layer, we derive the weight prediction set $W={[{w}_{i}]}_{i=1}^{K}$.
\begin{equation}
\widehat{S}_{w}^{i} =\mathcal{M}(\displaystyle\sum_{j=1}^{K}{w}_{j}\cdot{S}_{v}^{j}) ,
\end{equation}
where the $\mathcal{M}(\cdot)$  is a lightweight projection head designed to perform dimensionality transformation on the re-weighted priors, the $\widehat{S}_{w}^{i}\in {R}^{{C}^{i}\times{H}^{i}\times{W}^{i}}$ is the re-weighted priors for $i$-th encoder or decoder layer.

\begin{figure*}[ht]
\centering 
\includegraphics[width=0.9\linewidth]{figs/fig3_6.pdf}
% \vspace{1em}
\caption{The framework of our VarFormer includes two training stages. 
{\bf Stage 1:} To preserve the inherent knowledge of VAR and further enhance its adaptive distribution alignment capability, we freeze the VAR and integrate an Adapter to deliberately reduce the distance between the multi-scale latent representations of clean and degraded images, thereby obtaining multi-scale distribution alignment embedding ${S}_{v}$. 
{\bf Stage 2:} To adaptively extract valuable VAR scale priors for input-specific degradation type, the Degradation-Aware Enhancement (DAE) module is designed to distinguish different degradation types and integrate relevant priors, thus providing effective scale-aware alignment prior for the restoration process. 
Furthermore, the Adaptive Feature Transformation (AFT) module integrates the VAR scale priors into the image restoration network to guide the elimination of degradation.
} \label{fig3}
\end{figure*}

Furthermore, we must consider that not every region in a degraded image may need to undergo the transition from the degraded domain to the clean domain. To adjust the guidance strength of the priors according to the degradation conditions of different regions, inspired by ~\cite{liu2024hcanet}, we facilitate interaction between ${F}_{e/d}^{i} \in {R}^{{C}^{i}\times{H}^{i}\times{W}^{i}}$ and $\widehat{S}_{w}^{i}$ at the channel level, enabling them to better capture long-range dependencies. After processing through a lightweight network, we obtain region-specific fusion weights ${w}_{1}^{g}$ and ${w}_{2}^{g}$ for  ${F}_{e/d}^{i}$ and $\widehat{S}_{w}^{i}$, respectively. Ultimately, the feature ${F}_{{g}_{e/d}}^{i}\in {R}^{{C}^{i}\times{H}^{i}\times{W}^{i}}$ is derived by summing ${F}_{e/d}^{i}$ and $\widehat{S}_{w}^{i}$, each multiplied by their respective weights:
\begin{equation}
% \begin{aligned}
{w}_{1}^{g}, {w}_{2}^{g} = Softmax(Conv(RSTBs(Concat({F}_{e/d}^{i},\widehat{S}_{w}^{i})))) \nonumber
\end{equation}
\begin{equation}
{F}_{{g}_{e/d}}^{i} = {F}_{e/d}^{i} \times {w}_{1}^{g} + \widehat{S}_{w}^{i} \times {w}_{2}^{g} 
% \end{aligned}
\end{equation}
where $Concat(\cdot)$ refers to the concatenation operation, the $RSTBs(\cdot)$ means a series of Residual Swin-Transformer Blocks, the $Conv(\cdot)$ represents the convolutional layer and the $Softmax(\cdot)$ means the Softmax activation layer.


{\bf Adaptive Feature Transformation (AFT)} (Train in Stage 2).
We employ Adaptive Feature Transformation (AFT) to alleviate structural warping and textural distortion resulting from the fusion of high-quality priors and low-quality degraded features. Unlike standard cross-attention, we introduce a low-dimensional intermediate feature $M$ that aggregates both ${F}_{{g}_{e/d}}^{i}$ and ${F}_{e/d}^{i}$ as the mediator for similarity comparison, as illustrated in Fig.~\ref{fig3}. Specifically, given the intermediate feature ${F}_{e/d}^{i}$ and the degradation-aware enhanced feature ${F}_{{g}_{e/d}}^{i}$, we obtain the bridging feature ${F}_{{m}_{e/d}}^{i}=Concat({F}_{{g}_{e/d}}^{i},{F}_{e/d}^{i})$, where ${F}_{{m}_{e/d}}^{i}\in {R}^{{2C}^{i}\times{H}^{i}\times{W}^{i}}$. Then, ${F}_{e/d}^{i}$ is projected into the query $Q={W}_{q}{F}_{e/d}^{i}$, ${F}_{{m}_{e/d}}^{i}$ is projected into the mediator $M={W}_{m}{F}_{{m}_{e/d}}^{i}$, and ${F}_{{g}_{e/d}}^{i}$ is projected into the key $K={W}_{k}{F}_{{g}_{e/d}}^{i}$ and value $V={W}_{v}{F}_{{g}_{e/d}}^{i}$. Here, ${W}_{m}$, ${W}_{q}$, ${W}_{k}$, ${W}_{v}$ are all implemented using convolutional kernels. Formally, the transformation process is defined by the following equations:

\begin{equation}
{F}_{in}^{i+1}={A}_{q,m}\cdot({A}_{m,k}\cdot V) + {F}_{e/d}^{i}\nonumber
\end{equation}
\begin{equation}
{A}_{q,m}=Softmax(Q\cdot {M}^{T}/\sqrt{d})\
\end{equation}
\begin{equation}
{A}_{m,k}=Softmax(M\cdot {K}^{T}/\sqrt{d})\nonumber
\end{equation}
where $L \ll  H$, ${A}_{q,m} \in {R}^{H\times L} $ and ${A}_{m,k} \in {R}^{L\times H} $ denotes the attention map between the query-mediator pair and mediator-key pair.

In addition, to address the inherent loss of detail and texture due to downsampling operations, we propose an adaptive mix-up skipping to integrate encoder features into the decoder, thereby mitigating information loss:
\begin{equation}
{F}_{d}^{i} = \sigma ({\theta }_{i})\times \widehat{F}_{d}^{i} + (1-\sigma ({\theta }_{i}))\times{F}_{e}^{i}
\end{equation}
where ${\theta }_{i}$ represents a learnable coefficient, $\sigma$ denotes the sigmoid operator, and $\widehat{F}_{d}^{i}\in {R}^{{C}^{i}\times{H}^{i}\times{W}^{i}}$ is the output of residual blocks of the $i$-th layer.


\begin{figure*}[!h]
\centering 
\includegraphics[width=0.95\linewidth]{figs/rain.pdf}
\caption{Visual comparison with state-of-the-art methods on image deraining task. Please zoom in for details.} 
\label{fig:rain}
\end{figure*}

\begin{figure*}[]
\centering 
\includegraphics[width=0.95\linewidth]{figs/tolet.pdf}
\caption{The visualization results of zero-shot generalization in real-world TOLED dataset. Please zoom in for details.} 
\label{fig:tolet}
\end{figure*}

\subsection{Training Objectives}


{\bf Feature Matching Loss.} The goal of the first stage is to further enhance the distribution alignment capability of VAR. Consequently, we design the Feature Matching Loss to reduce the feature discrepancies between degraded images and clean images, which can be formulated as follows:

\begin{equation}
{\mathcal{L}}_{fema} = \displaystyle\sum_{i=1}^{K}-{s}_{i}log(\widehat{s}_{i}) + {\left \| 
 {F}_{a}-sg({F}_{{e}_{gt}}^{q}) \right \|}_{2}^{2}
\end{equation}
where ${s}_{i}$ is the  ground-truth of $i$-th scale latent representation, $\widehat{s}_{i}$ is the output of VAR Transformer, and ${F}_{a}$ is the output of Adapter.

\noindent {\bf Reconstruction Loss.} This loss is utilized in the second training stage, with the purpose of ensuring that the restored image possesses a completed structure and impressing visual pleasure. It consists of two components: the PSNR loss and the perceptual loss. It is formulated as follows:
\begin{equation}
{\mathcal{L}}_{rec} = {-PSNR({I}_{gt},{I}_{rec}) + {\left \| \psi ({I}_{gt})-\psi ({I}_{rec})\right \|}_{2}^{2}}
\end{equation}
where $\psi(\cdot)$ indicates  the pre-trained VGG19 network.



































==> 4_Experiments.tex <==
\section{Experiments}
\label{sec:exp}


In this section, we first clarify the experimental settings of our method, and then present qualitative and quantitative results compared with the state-of-the-art methods on all-in-one and zero-shot tasks. Moreover, we also conduct extensive ablations to verify the effectiveness of our method.


% % -------------------------------------------------------

\begin{table*}[h]
\centering
\caption{Quantitative comparison with state-of-the-art task-specific methods and universal methods on image deraining, low-light image enhancement, motion deblurring and image dehazing tasks. 
% The best and the second best results are marked in bold and underlined, respectively.
}
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{cccccccccc}
\toprule

\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Year}}} & \multicolumn{2}{c|}{\textbf{Deraining (5sets)}}    & \multicolumn{2}{c|}{\textbf{Deblurring}}    & \multicolumn{2}{c|}{\textbf{Enhancement}}    & \multicolumn{2}{c}{\textbf{Dehazing}}     \\

\multicolumn{1}{l|}{}                                 & \multicolumn{1}{c|}{}                               & PSNR↑        & \multicolumn{1}{c|}{SSIM↑}        & PSNR↑     & \multicolumn{1}{c|}{SSIM↑}     & PSNR↑      & \multicolumn{1}{c|}{SSIM↑}     & PSNR↑              & \multicolumn{1}{c}{SSIM↑}                \\ \midrule
\multicolumn{10}{l}{\textbf{Task-specific Method}}                                                                                                                                                                                                                                          \\ \midrule
\multicolumn{1}{c|}{SwinIR~\cite{liang2021swinir}}                           & \multicolumn{1}{l|}{2021}                           & -           & \multicolumn{1}{c|}{-}           & 24.52    & \multicolumn{1}{c|}{0.773}    & 17.81     & \multicolumn{1}{c|}{0.723}    & 21.50      & \multicolumn{1}{c}{0.891}                  \\

\multicolumn{1}{c|}{MIRNet~\cite{zamir2020learning}}                        & \multicolumn{1}{l|}{2022}                           & -           & \multicolumn{1}{c|}{-}           & 26.30    & \multicolumn{1}{c|}{0.799}    & 24.74     & \multicolumn{1}{c|}{0.851}    & 24.03      & \multicolumn{1}{c}{0.927}                  \\
\multicolumn{1}{c|}{Restormer~\cite{zamir2022restormer} }                       & \multicolumn{1}{l|}{2022}                           & 33.96       & \multicolumn{1}{c|}{0.935}       & 32.92    & \multicolumn{1}{c|}{0.961}    & 20.41     & \multicolumn{1}{c|}{0.806}    & 30.87         & \multicolumn{1}{c}{0.969}               \\
\multicolumn{1}{c|}{MAXIM~\cite{tu2022maxim}}                            & \multicolumn{1}{l|}{2022}                           & 33.24       & \multicolumn{1}{c|}{0.933}       & 32.86    & \multicolumn{1}{c|}{0.940}    & 23.43     & \multicolumn{1}{c|}{0.863}    & -         & \multicolumn{1}{c}{-}                      \\
\multicolumn{1}{c|}{RDDM~\cite{liu2024residual}}                             & \multicolumn{1}{l|}{2023}                           & 30.65       & \multicolumn{1}{c|}{0.901}       & 28.83    & \multicolumn{1}{c|}{0.846}    & 24.22     & \multicolumn{1}{c|}{0.889}    & 30.76       & \multicolumn{1}{c}{0.943}                  \\ \midrule
\multicolumn{10}{l}{\textbf{Universal Method}}                                                                                                                                                                                                                                              \\ \midrule
\multicolumn{1}{c|}{AirNet~\cite{Li2022AllInOneIR}}                            & \multicolumn{1}{l|}{2022}                           & 25.44       & \multicolumn{1}{c|}{0.743}       & 27.14    & \multicolumn{1}{c|}{0.832}    & 18.49     & \multicolumn{1}{c|}{0.767}    & 25.48      & \multicolumn{1}{c}{0.944}                 \\
\multicolumn{1}{c|}{Painter~\cite{wang2023images} }                          & \multicolumn{1}{l|}{2022}                           & 29.49       & \multicolumn{1}{c|}{0.868}       & -        & \multicolumn{1}{c|}{-}        & 22.40     & \multicolumn{1}{c|}{0.872}    & -       & \multicolumn{1}{c}{-}                         \\
\multicolumn{1}{c|}{IDR~\cite{zhang2023ingredient}}                              & \multicolumn{1}{l|}{2023}                           & 30.87           & \multicolumn{1}{c|}{0.906}           & 27.94    & \multicolumn{1}{c|}{0.848}    & 22.32     & \multicolumn{1}{c|}{0.836}    & 25.33      & \multicolumn{1}{c}{0.945 }                \\
\multicolumn{1}{c|}{DA-CLIP~\cite{luo2023controlling}}                        & \multicolumn{1}{l|}{2023}                           & 28.75       & \multicolumn{1}{c|}{0.844}       & 26.24    & \multicolumn{1}{c|}{0.801}    & 24.27     & \multicolumn{1}{c|}{0.885}    & 31.42       & \multicolumn{1}{c}{0.941}                 \\
\multicolumn{1}{c|}{Prompt-IR~\cite{potlapalli2306promptir}}                        & \multicolumn{1}{l|}{2023}                           & 29.44       & \multicolumn{1}{c|}{0.848}       & 27.31    & \multicolumn{1}{c|}{0.834}    & 22.95     & \multicolumn{1}{c|}{0.844}    & 32.17       & \multicolumn{1}{c}{0.953}                  \\
\multicolumn{1}{c|}{DiffUIR~\cite{zheng2024selective}}                        & \multicolumn{1}{l|}{2024}                           & 31.14       & \multicolumn{1}{c|}{0.907}       & 29.88    & \multicolumn{1}{c|}{0.874}    & 25.02     & \multicolumn{1}{c|}{0.901}    & 32.74       & \multicolumn{1}{c}{0.944}                \\

\rowcolor[HTML]{E2E2E2} \multicolumn{1}{c|}{\textbf{VarFormer}}               & \multicolumn{1}{c|}{-}                              &{\color{red}31.33}             & \multicolumn{1}{c|}{{\color{red}0.913}}            &{\color{red}30.99}          & \multicolumn{1}{c|}{{\color{red}0.956}}         &{\color{red}25.13}           & \multicolumn{1}{c|}{{\color{red}0.917}}         &{\color{red}32.96}                   & \multicolumn{1}{c}{{\color{red}0.956}}                       \\ \bottomrule
\end{tabular}}
\label{tab:aio}
\end{table*}



\begin{table}[h]
\centering
\caption{Quantitative results of Gaussian denoising on BSD68,
Urban100 and Kodak24 datasets in terms of PSNR↑.}
\setlength{\tabcolsep}{0.3mm}
\fontsize{9}{12}\selectfont{
\begin{tabular}{c|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{BSD68}} & \multicolumn{3}{c|}{\textbf{Urban100}} & \multicolumn{3}{c}{\textbf{Kodak24}} \\
                                 & $\sigma$=15         & $\sigma$=25         & $\sigma$=50        & $\sigma$=15          & $\sigma$=25          & $\sigma$=50         & $\sigma$=15         & $\sigma$=25         & $\sigma$=50         \\ \midrule
HINet~\cite{chen2021hinet}                            & 33.72      & 31.00      & 27.63     & 33.49       & 30.94       & 27.32      & 34.38      & 31.84      & 28.52      \\
MPRNet~\cite{Zamir2021MultiStagePI}                            & 34.01      & 31.35      & 28.08     & 34.13       & 31.75       & 28.41      & 34.77      & 32.31      & 29.11      \\
MIRV2~\cite{zamir2020learning}                         & 33.66      & 30.97      & 27.66     & 33.30       & 30.75       & 27.22      & 34.29      & 31.81      & 28.55      \\
SwinIR~\cite{liang2021swinir}                           & 33.31      & 30.59      & 27.13     & 32.79       & 30.18       & 26.52      & 33.89      & 31.32      & 27.93      \\
Restormer~\cite{zamir2022restormer}                        & 34.03      & 31.49      & 28.11     & 33.72       & 31.26       & 28.03      & 34.78      & 32.37      & 29.08      \\ \midrule
AirNet~\cite{Li2022AllInOneIR}                          & 33.49      & 30.91      & 27.66     & 33.16       & 30.83       & 27.45      & 34.14      & 31.74      & 28.59      \\
IDR~\cite{zhang2023ingredient}                                & 34.05      & 31.67      & 28.05     & 32.92       & 31.29       & 28.45      & 34.53      & 32.22      & 28.93      \\
DA-CLIP~\cite{luo2023controlling}   & 30.16      & 28.89      & 27.04     & 33.14       & 30.99       & 27.61     & 33.86     & 32.30      & 28.84      \\
Prompt-IR~\cite{potlapalli2306promptir} & 32.17      & 29.89      & 28.03     & 33.04       & 31.89       & 27.72     & 33.78     & 32.21      & 28.64      \\
DiffUIR~\cite{zheng2024selective}       & 33.86      & 30.88      & 26.63     & 32.19       & 29.65       & 25.87      & 33.24      & 30.70      & 27.19      \\
\rowcolor[HTML]{E2E2E2} VarFormer                        & {\color{red}34.11}      & {\color{red}31.85}      & {\color{red}28.23}     & {\color{red}33.13}       & {\color{red}31.94}       & {\color{red}28.96}      & {\color{red}34.73}      & {\color{red}32.40}      & {\color{red}29.02}            \\ \bottomrule
\end{tabular}
}
\label{tab:syn_noise}
\end{table}

%-------------------------------------------------------------

\begin{table}[!h]
\centering
\caption{Quantitative results of Real image denoising on SIDD in terms of PSNR↑ and SSIM↑.}
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{c|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{SIDD}} \\
                                 & PSNR↑                     & SSIM↑                    \\ \midrule
MPRNet~\cite{Zamir2021MultiStagePI}                            & 39.71                    & 0.958                   \\
Uformer~\cite{Wang2021UformerAG}                          & 39.89                    & 0.961                   \\
Restormer~\cite{zamir2022restormer}                        & 40.02                    & 0.967                   \\
ART~\cite{zhang2022accurate}                              & 39.99                    & 0.964                   
% \\
%                                  &                          &                         
                                 \\ \midrule
AirNet~\cite{Li2022AllInOneIR}                          & 38.32                    & 0.945                   \\
Prompt-IR~\cite{potlapalli2306promptir}                         & 39.52                    & 0.954                   \\
DA-CLIP~\cite{luo2023controlling}                          & 34.04                    & 0.824                   \\
IDR~\cite{zhang2023ingredient}                          & 39.74                    & 0957                    \\
MPerceiver~\cite{ai2024multimodal}                       & 39.96                    & 0.959                   \\
Painter~\cite{wang2023images}                          & 38.88                    & 0.954                   \\
\rowcolor[HTML]{E2E2E2} VarFormer                        &{\color{red}40.13}                          &{\color{red}0.978}                         \\ \bottomrule
\end{tabular}}
\label{tab:real_noise}
\end{table}



\subsection{Experimental Settings }
{\bf Datasets.} (1) All-in-one :  We train a unified model to solve 6 IR tasks, including deraining, dehazing, low-light enhancement, motion deblurring, Gaussian denoising and real image denoising. For deraining, We adopt Rain13K~\cite{Fu2016ClearingTS,Li2018RecurrentSC,Li2016RainSR,Luo2015RemovingRF,Yang2019SingleID} for training, and 5 datasets for testing, including Rain100L~\cite{Yang2016DeepJR}, Rain100H~\cite{Yang2016DeepJR}, Test100~\cite{Zhang2017ImageDU}, Test1200~\cite{Zhang2018DensityAwareSI} and Test2800~\cite{Fu2017RemovingRF}. For dehazing, the RESIDE~\cite{li2018benchmarking} dataset is used as the benchmark. As the real-world fog condition is outdoor, we only train and test on the outdoor part. For low-light enhancement, LOL dataset~\cite{Wei2018DeepRD} is adopted. For motion deblurring, we adopt GoPro~\cite{Nah2016DeepMC} dataset for training and testing.
For Gaussian denoising, BSD400~\cite{martin2001database} and WED~\cite{ma2016waterloo} are used for training and BSD68~\cite{Martin2001ADO}, Urban100~\cite{Huang2015SingleIS}, Kodak24~\cite{franzen1999kodak} for testing.
For real image denoising, We use SIDD~\cite{abdelhamed2018high} datasets as the benchmark for training and testing.
(2) Zero-shot: we utilize TOLED~\cite{zhou2021image} and POLED ~\cite{zhou2021image} for under-display camera (UDC) IR.



{\bf Evaluation Metrics.} 
To evaluate the restoration performance, we adopt Signal to Noise Ratio (PSNR), Structural Similarity (SSIM) and Learned Perceptual Image Patch Similarity (LPIPS)~\cite{zhang2018unreasonable}. 
We emphasize the performance of the universal methods, with the best results shown in {\color{red}red}.


{\bf Implementation Details.} 
We adopt the Adam optimizer~\cite{Kingma2014AdamAM}(${\beta }_{1}=0.9$, ${\beta}_{2}=0.999$) with the initial learning rate 1e-4 gradually reduced to 1e-6 with cosine annealing to train our model.We random crop $256\times256$ patch from original image as network input after data augumentation. As the data size varies greatly from task to task,
we set the weight of each task in one batch as 0.3 for dehazing, 0.1 for low-light, 0.2 for deraining, 0.2 for Gaussian denoising,0.1 for real image denoising, and 0.1 for motion deblurring.



\subsection{All-in-One Restoration}
We compare VarFormer with both task-specific and universal methods. To ensure a fair evaluation, we train all-in-one models from scratch using our training strategy. The quantitative results are presented in ~\cref{tab:aio,tab:syn_noise,tab:real_noise}, where it can be observed that VarFormer demonstrates superior performance across all 6 tasks. Notably, in low-light enhancement and dehazing tasks, VarFormer's performance with the all-in-one training strategy even surpasses that of task-specific methods, highlighting its exceptional capabilities. We also provide visual comparisons with other state-of-the-art universal methods, as shown in Fig.~\ref{fig:rain}, with more results available in the supplementary material. It is evident that, compared to other universal methods, VarFormer yields more steady results in all image restoration tasks.
%  and ~\ref{fig:low}




\subsection{Zero-shot Results}
In Tab.~\ref{tab:zero-shot}, we present the generalization performance of various methods on unseen tasks without fine-tuning. Specifically, high-resolution images captured under under-display camera (UDC) systems often suffer from various types of degradations due to the point spread function and lower light transmission rate, posing challenges for the prediction of restoration models. Encouragingly, our VarFormer achieves state-of-the-art performance. For instance, as shown in Fig.~\ref{fig:tolet}, compared to other universal methods, our approach effectively addresses blurring.

\begin{table}[!h]
\centering
\caption{Quantitative results of unknown tasks (under-display
camera image restoration) on TOLED and POLED datasets.}
\setlength{\tabcolsep}{0.1mm}
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{TOLED}} & \multicolumn{3}{c}{\textbf{POLED}} \\
                                 & PSNR↑       & SSIM↑       & LPIPS↓     & PSNR↑       & SSIM↑      & LPIPS↓     \\ \midrule
NAFNet~\cite{chen2022simple}                           & 26.89      & 0.774      & 0.346     & 10.83      & 0.416     & 0.794     \\
HINet~\cite{chen2021hinet}                            & 13.84      & 0.559      & 0.448     & 11.52      & 0.436     & 0.831     \\
MPRNet~\cite{Zamir2021MultiStagePI}                           & 24.69      & 0.707      & 0.347     & 8.34       & 0.365     & 0.798     \\
DGUNet~\cite{mou2022deep}                           & 19.67      & 0.627      & 0.384     & 8.88       & 0.391     & 0.810     \\
MIRV2~\cite{zamir2020learning}                         & 21.86      & 0.620      & 0.408     & 10.27      & 0.425     & 0.722     \\
SwinIR~\cite{liang2021swinir}                           & 17.72      & 0.661      & 0.419     & 6.89       & 0.301     & 0.852     \\
Restormer~\cite{zamir2022restormer}                        & 20.98      & 0.632      & 0.360     & 9.04       & 0.399     & 0.742     \\ \midrule
TAPE~\cite{liu2022tape}                             & 17.61      & 0.583      & 0.520     & 7.90       & 0.219     & 0.799     \\
AirNet~\cite{Li2022AllInOneIR}                         & 14.58      & 0.609      & 0.445     & 7.53       & 0.350     & 0.820     \\
DA-CLIP~\cite{luo2023controlling}                               & 15.74      & 0.606      & 0.472     & 14.91      & 0.475     & 0.739     \\
IDR~\cite{zhang2023ingredient}                              & 27.91      & 0.795      & 0.312     & 16.71      & 0.497     & 0.716     \\
DiffUIR~\cite{zheng2024selective}                          & 29.55      & 0.866      & 0.281     & 15.62      & 0.424     & {\color{red}0.505}     \\
\rowcolor[HTML]{E2E2E2} VarFormer                        & {\color{red}30.61}      & {\color{red}0.887}      & {\color{red}0.275}     & {\color{red}16.63}      & {\color{red}0.499}     & 0.605           \\ \bottomrule
\end{tabular}
\label{tab:zero-shot}
\end{table}




\subsection{Abalation Studies}
In this section, we perform a series of ablation studies to better the effectiveness of our designs. In Tab.~\ref{tab:alab_components}, we conducte ablation studies on the design of key components, including the adaptive mix-up skip that integrates encoder features into the decoder, the adapter that addresses the domain shift issue when using pre-trained VAR on degraded datasets, and the DAE and AFT modules responsible for generating and fusing multi-scale distribution alignment priors. We evaluate the performance based on the average performance across six tasks. The results indicate a gradual improvement with the addition of each component and a corresponding decline when each component is removed, underscoring the effectiveness of each module.


 \begin{figure}[!ht]
\centering 
{\includegraphics[width=\linewidth]{figs/aba_DAE.pdf}}

\caption{The training trajectory using different number of DAE.} 
\label{fig:ab_DAE}
\end{figure} 

\begin{table}[!h]
% \footnotesize
% \setlength\tabcolsep{2pt} 
\centering
\caption{Ablation experiments on the components design. }
% \vspace{-0.2cm}
\setlength{\tabcolsep}{1.7mm}{
\begin{tabular}{c|cccc|cc}
\toprule
Exp. & skip       & adapter    & AFT        & DAE        & PSNR↑ & SSIM↑ \\ \midrule
a      &            &            &            &            & 27.54     & 0.841    \\
b      &            & \checkmark & \checkmark & \checkmark & 29.37     &  0.905     \\
c      & \checkmark &            & \checkmark & \checkmark &  29.51    & 0.917     \\
d      & \checkmark & \checkmark &            & \checkmark &  29.29    &  0.891    \\
e      & \checkmark &            & \checkmark &            &   28.98   &  0.867   \\
f      & \checkmark & \checkmark & \checkmark & \checkmark & 29.66     & 0.926     \\ \bottomrule

\end{tabular}}
\label{tab:alab_components}
% \vspace{0.5em}
\end{table}

\begin{table}[!h]
% \footnotesize
% \setlength\tabcolsep{2pt} 
\centering
\caption{Ablation experiments on the DAE number.}
% \vspace{-0.2cm}
% \setlength{\tabcolsep}{0.7mm}
\begin{tabular}{c|cccc|cc}
\toprule
\multirow{2}{*}{Exp.} & \multicolumn{4}{c|}{DAE}                                              & \multirow{2}{*}{PSNR↑} & \multirow{2}{*}{SSIM↑} \\ \cline{2-5}
                        & all                  & skip1      & skip2      & w/o &                      &                       \\ \midrule
a                       &                                    &            &            & \checkmark     & 28.98                       & 0.867                      \\
b                       &                                    &            & \checkmark &      &  29.29                     &    0.883                   \\
c                       &                                    & \checkmark &            &      &  29.49                     &    0.902                   \\
d       &\checkmark                 &            &            &      & 29.66                      & 0.926                      \\ \bottomrule
\end{tabular}
\label{tab:alab_AFT}
\vspace{-0.1cm}
\end{table}
Additionally, we explored the influence of the guidance strength of VAR multi-scale priors on restoration tasks by altering the quantity of DAE modules. The results from Tab.~\ref{tab:alab_AFT} indicate a positive correlation between model performance and the guidance strength provided by VAR priors. 
This discovery indicates that the multi-scale priors within VAR exhibit notable effectiveness in directing the optimization trajectory of intricate multi-task restoration endeavors, effectively steering the model towards enhancing performance.
The training trajectories illustrated in Fig.~\ref{fig:ab_DAE} also support this conclusion, indicating that the integration of DAE modules can accelerate the model's convergence.



==> 5_Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we investigate the multi-scale representations of the generative model VAR and reveal its endogenous multi-scale priors. As the autoregressive scales evolve, it transitions from capturing global color information to focusing on fine-grained details and adaptively aligns the input with clean images scale by scale. Furthermore, we propose the VarFormer framework integrated with multi-scale priors for multiple degradation restoration. Extensive experiments on various image restoration tasks demonstrate the effectiveness and generalization of our method.
